Advances in diffraction of subnuclear waves

In this review, we present and discuss the most recent results on inclusive and exclusive diffractive processes at HERA and Tevatron colliders. Measurements from fixed target experiments at HERMES and Jefferson laboratory are also reviewed. The complementarity of all these results is analysed in the context of perturbative QCD and new challenging issues in nucleon tomography are studied. A first understanding of how partons are localised in the nucleon to build orbital momenta can be addressed with these experimental results. Some prospects are outlined for new measurements in fixed target kinematic, at Jefferson laboratory and CERN, at COMPASS, or at the LHC. Of special interest is the exclusive (coherent) production of Higgs boson and heavy objects at the LHC. Based on the present knowledge, some perspectives are presented in this direction.

==> conclusion.tex <==
Many aspects of diffraction in ep collisions can be successfully 
described in QCD if a hard scale is
present. A key to this success are factorization theorems, which render parts of the dynamics 
accessible to calculation in perturbation theory. The remaining 
non-perturbative quantities, namely diffractive
PDFs and generalized parton distributions, can be extracted from 
measurements and contain specific
information about small-x partons in the proton that can only be obtained in diffractive processes. To
describe hard diffractive hadron-hadron collisions is more challenging since factorization is broken by
rescattering between spectator partons. 
These rescattering effects are of interest in their own right 
because of their intimate relation with multiple scattering effects, which at 
LHC energies are expected to be
crucial for understanding the structure of events in hard collisions. 
A combination of data on inclusive
and diffractive ep scattering hints at the onset of parton saturation at 
HERA, and the phenomenology
developed there is a helpful step towards understanding high-density 
effects in hadron-hadron collisions.
%%%%%%%%%%
In this talk I have reviewed progress in selected areas connected with
generalized parton distributions.  There are many interesting aspects
discussed in the recent literature which I could not cover for reasons
of time.  Among these are studies of GPDs in dynamical models, GPDs of
nuclei, production of exotic mesons, GPDs for hadron-photon and
baryon-meson transitions, hard exclusive processes at large $s$ and
$t$, and possibilities to study GPDs in neutrino-nucleon scattering
with future high-intensity neutrino beams.

To summarize, there has been important technical progress in the
description of hard exclusive processes, with full NLO results in
$\alpha_s$ available for most relevant channels, partial NNLO results
for Compton scattering, and a better understanding of the scale
evolution of GPDs.  These advances remain to be fully implemented in
the analysis of data, but existing studies have in particular shown
the high sensitivity of vector meson production to the generalized
gluon distribution, even at the moderate $x$ accessible in
fixed-target experiments.

Through the impact parameter representation, GPDs provide information
on the spatial distribution of partons in a hadron, and a number of
studies have turned this concept into quantitative information.
Phenomenological analysis of elastic form factors, as well as results
from lattice QCD show that the average impact parameter of valence
quarks strongly decreases with their momentum fraction in the proton.
The proton helicity-flip distribution $E^q$ has connections with two
crucial aspects of spin physics: transverse polarization effects and
the orbital angular momentum $L^q$ carried by quarks in the nucleon.
First steps have been taken towards a quantitative understanding of
$L^q$.  The present picture---suggested both by lattice results and
model-dependent analysis of experimental data---is that for individual
quark flavors $L^q$ may be substantial, but that when summed over
flavors the orbital angular momentum carried by \emph{valence} quarks
contributes little to the nucleon spin.  The proton spin puzzle thus
remains a puzzle.

%%%%%%%%
In this  review,
the idea is to cover the main advances in (hard) diffraction
during  the last years for which our impact was significant,
either from the experimental side or, when possible,
from the interpretation border.

Concerning inclusive diffraction, we have discussed 
the main areas in which we have contributed: measurements, 
extraction of diffractive PDFs, HERA results put in 
perspective with Tevatron observables, 
prospectives for LHC. 
We have discussed in length
a very important aspect that makes diffraction in DIS  so
interesting at low $x_{Bj}$: its interpretation in the
dipole formalism and its connection
to saturation effects. Indeed, diffraction in DIS has appeared as
a well suited process to analyse staturation effects 
at large gluon density in the proton. In the dipole model,
it takes a simple and luminous form, with the introduction of
a saturation scale $Q_s$. Diffraction is then dominated
by dipoles of size $r \sim 1/Q_s$, which makes naturally diffractive
processes sensitive to saturation
effects. In particular, it provides a simple 
 explanation of the
constance of the ratio of diffractive to total cross sections
as a function of $W$ (at fixed $Q^2$ values).

Concerning exclusive processes and DVCS, our contributions have
been dominant in the experimental measurements, in particular with
 determinations of DVCS cross sections and their dependences in $t$  
(analysing H1 data). These measurements have allowed us to merge 
DVCS with other exculsive reactions at HERA
and to provide a common perspective for
all processes. For example, with results of the energy dependence 
power, $\delta(Q^2)$ with $\sigma \sim W^\delta$,
and of the exponential $t$ slope, $b(Q^2,W)$, with $d\sigma/dt \sim e^{-b|t|}$. 
A unified picture is clear. 
Either from the dipole approach of in the GPDs formalism.
Of course, both approaches include the same main physics features, either in
the dipole cross section (dipole formalism) of in the initial 
conditions (GPDs formalism). A specific interest for DVCS is important:
DVCS is certainly the best 
candidate for a (pure) description with GPDs, avoiding
unknowns from the vector meson wave functions.
Along the years and analysis,
we have focused our attention,
not only on HERA results but also on 
all the other experiments measuring  DVCS or excluisve (hard)
particle production.
This perspective gives much more insight into 
the definition of  key elements for the future.
This explains why we have been interested in the COMPASS project for 
measuring DVCS at CERN after 2010. The expected kinematic domain is
lying between H1/ZEUS and HERMES/JLab experiments. 
It gives promising perspectives in understanding the 
transition from low to large $x_{Bj}$
for many observables.
Our experimental work on 
 the impact parameter dependence of parton distributions
 (also as a function of
$x_{Bj}$) is of fundamental interest. It provides 
a completely new information on the spatial extension of partons
inside the proton (or hadrons). We have
explained the new insights of such analysis.
For example, our measurements have established that
small $x_{Bj}$ partons
of the nucleon contribute more for large values of $b$.
Also, shadowing of small $x_{Bj}$ parton distributions, 
is probably stronger at small values
of $b$ since partons in the geometric center 
of the nucleon are more effectively
shielded by the surrounding partons.
These and many other results and intuitive pictures 
for the parton structure of
hadrons give rise to (first) predictions for the impact 
parameter dependence of GPDs
that reflect the underlying microscopic dynamics. 

Of course, we do not forget that the dependence of GPDs on three
kinematical variables, and the number of distributions describing
different helicity combinations present a considerable complexity.  In
a sense this is the price to pay for the amount of physics information
encoded in these quantities.  It is however crucial to realize that
for many important aspects one need not fully disentangle this
complexity.  The relation of longitudinal and transverse structure
of partons in a nucleon, or of nucleons in a nucleus, can be studied
quantitatively from the distribution in the two external kinematical
variables $\xi$ and $t$, even if the deconvolution of the loop
integral over the variable $x$ is not performed.  

